Multi-Perspective Abstractive Answer Summarization

Community Question Answering (CQA) forums such as Stack Overflow and Yahoo! Answers contain a rich resource of answers to a wide range of questions. Each question thread can receive a large number of answers with different perspectives. The goal of multi-perspective answer summarization is to produce a summary that includes all perspectives of the answer. A major obstacle for multi-perspective, abstractive answer summarization is the absence of a dataset to provide supervision for producing such summaries. This work introduces a novel dataset creation method to automatically create multi-perspective, bullet-point abstractive summaries from an existing CQA forum. Supervision provided by this dataset trains models to inherently produce multi-perspective summaries. Additionally, to train models to output more diverse, faithful answer summaries while retaining multiple perspectives, we propose a multi-reward optimization technique coupled with a sentence-relevance prediction multi-task loss. Our methods demonstrate improved coverage of perspectives and faithfulness as measured by automatic and human evaluations compared to a strong baseline.

==> prev/misc_save.tex <==
% SECTION: old text re data part
% % \par
% We found that a BART model trained on CQASumm was almost entirely extractive, likely due to how the dataset was filtered. We found fewer hallucinations when the model was trained on the dataset filtered by entailment and fewer with the model filtered according to named entities. For these models, the types of hallucinations found were sometimes plausible answers, even though the answer was not stated directly in the source documents. We show a comparison of our data and some characteristics to \ref{tab:statistics}. 
% \subsection{Alternative Pipeline}
% We explore an alternative dataset creation pipeline centered on sub-aspects of summarization as detailed in \citet{jung-etal-2019-earlier}. This paper introduces quantitative notions of position, importance and diversity in existing summarization datasets. Importance is defined by correlation of dimension-reduced sentence embeddings. Diversity is defined by coverage in a convex hull. Specifically, we use their N-nearest formulation of importance, which calculates an averaged Pearson correlation between one sentence and the rest for the source sentence vector representations and picks the summaries with the highest averaged correlations. For diversity we make use of their ConvexFall algorithm which prunes redundant sentences from those chosen by the convex-hull search. We first extract the 10 most important sentences and then use the ConvexFall algorithm to prune sentences, keeping a max of 4 sentences (as this was the average number of sentences in our original pipeline). We find fairly similar trends for the two datasets in terms of statistics and baselines (this pipeline vs our original pipeline); length of 69 vs 75, novel unigrams 0.37 vs 0.34, repeated unigrams (0.22 vs 0.20). The BART baseline trained and validated on this dataset has a ROUGE-1 of 0.344 vs 0.325 for the model trained and validated on our data. However, running the model on this pipeline data and using the validation data created in our pipeline returns very similar ROUGE scores. 




% SECTION: misc old tables
% \newcommand{\DatasetComparison}{
%  \begin{table*}[t]
% \centering
% \small
% \begin{tabular}{c c c c c c } \Xhline{2\arrayrulewidth}
%              \textbf{Dataset} & \textbf{Novel unigrams} &  \textbf{Repeated unigrams}  &  \textbf{Oracle Extractive}  &  \textbf{Length}  &  \\ \Xhline{\arrayrulewidth}
%              Our Dataset & 0.24 & 0.20 &  40.22/10.93/35.52 & 75  \\ 
%             XSUM & 0.33 & 0.05 & 29.79/8.81/22.65 & 24 \\
%              CNN-DailyMail & 16.75 & 0.10 & 50.38/28.55/46.58 & 45.70 \\
%             \Xhline{2\arrayrulewidth}
% \end{tabular}
% \caption{Comparison of statistics between our proposed dataset pipeline and the standard XSum \cite{narayan-etal-2018-dont} and CNN-DailyMail \cite{nallapati-etal-2016-abstractive} summarization datasets. }
% \label{tab:statistics}
% \end{table*}
% }

% \newcommand{\BaselineResults}{
% \begin{table}[t!]
% \small
% \resizebox{\columnwidth}{!}{\begin{tabular}{|l|ccc|}
% \hline
%     \textbf{Method}   & \textbf{ROUGE-1}    & \textbf{ROUGE-2}    & \textbf{ROUGE-L}    \\ \hline \hline
% LexRank	&	26.65	&	4.84	&	23.32	\\
% TextRank	&	28.61	&	4.98	&	24.75	\\
% BertSum &	29.82	&	5.51	&	25.28	\\
% \hline
% \end{tabular}}
% \caption{ROUGE scores for baseline extractive models.}
% \label{tab:baseline_results}
% \end{table}
% }

